Adaptive Online Learning with Momentum for Contingency-based Voltage Stability Assessment

Voltage stability refers to the ability of a power system to maintain acceptable voltages among all buses under normal operating conditions and after a disturbance. In this paper, a measurement-based voltage stability assessment (VSA) framework using online deep learning is developed. Since the topology changes induced by transmission contingencies may significantly reduce the voltage stability margin, different network topologies under different operating conditions are involved in our training dataset. To achieve high accuracy in the training process, a gradient-based adaptive learning algorithms is adopted. Numerical results based on the NETS-NYPS 68-bus system demonstrate the effectiveness of the proposed VSA approach. Moreover, with the proximal function modified adaptively, the adaptive algorithm with momentum outperforms traditional nonadaptive algorithms whose learning rate is constant.

==> test_results_180803.tex <==
% Logged on %2018-08-03 17:42%
% **************** SGD ****************
% Epoch #4050. Train_acc: 0.91598141, Test_acc: 0.88916667, Time: 0.11679292, Loss:   0.19375611
%     >>> Completed! Training time: 515.29449916
% With  500 Epochs: train_acc: 0.87021809, test_acc: 0.83833333, loss: 0.30536175, cum_time:  63.6555s
% With 1000 Epochs: train_acc: 0.89274222, test_acc: 0.86833333, loss: 0.24591704, cum_time: 127.1331s
% With 1500 Epochs: train_acc: 0.90025027, test_acc: 0.88083333, loss: 0.22159493, cum_time: 190.6900s
% With 2000 Epochs: train_acc: 0.90990347, test_acc: 0.88916667, loss: 0.20357645, cum_time: 254.3229s
% With 2500 Epochs: train_acc: 0.91419378, test_acc: 0.89666667, loss: 0.19122954, cum_time: 317.9492s
% With 3000 Epochs: train_acc: 0.91633893, test_acc: 0.89500000, loss: 0.18922971, cum_time: 381.4749s
% With 3500 Epochs: train_acc: 0.91705399, test_acc: 0.89750000, loss: 0.18715755, cum_time: 445.0511s
% With 4000 Epochs: train_acc: 0.92742224, test_acc: 0.90333333, loss: 0.16381443, cum_time: 508.7789s
% Preset Learning Rate: 2e-05
% **************** SGD-m ****************
% Epoch #4050. Train_acc: 0.94708616, Test_acc: 0.92750000, Time: 0.16985393, Loss:   0.12239803
%     >>> Completed! Training time: 569.71606112
% With  500 Epochs: train_acc: 0.88022882, test_acc: 0.86916667, loss: 0.29656014, cum_time:  70.4134s
% With 1000 Epochs: train_acc: 0.91598141, test_acc: 0.90333333, loss: 0.20593812, cum_time: 140.6152s
% With 1500 Epochs: train_acc: 0.92348945, test_acc: 0.90916667, loss: 0.17546085, cum_time: 210.8664s
% With 2000 Epochs: train_acc: 0.92992492, test_acc: 0.91083333, loss: 0.15822170, cum_time: 281.3492s
% With 2500 Epochs: train_acc: 0.94923132, test_acc: 0.92416667, loss: 0.12083457, cum_time: 351.7973s
% With 3000 Epochs: train_acc: 0.94887379, test_acc: 0.92416667, loss: 0.11877385, cum_time: 421.8658s
% With 3500 Epochs: train_acc: 0.94637111, test_acc: 0.92500000, loss: 0.12578003, cum_time: 492.1229s
% With 4000 Epochs: train_acc: 0.94958885, test_acc: 0.92666667, loss: 0.11772717, cum_time: 562.4866s
% Preset Learning Rate: 2e-05
% **************** NAG ****************
% Epoch #4050. Train_acc: 0.93063997, Test_acc: 0.91166667, Time: 0.11788511, Loss:   0.15229238
%     >>> Completed! Training time: 517.49227738
% With  500 Epochs: train_acc: 0.90311048, test_acc: 0.88750000, loss: 0.21338746, cum_time:  63.7162s
% With 1000 Epochs: train_acc: 0.91455130, test_acc: 0.89333333, loss: 0.18619867, cum_time: 127.6456s
% With 1500 Epochs: train_acc: 0.92098677, test_acc: 0.90416667, loss: 0.17309516, cum_time: 191.6184s
% With 2000 Epochs: train_acc: 0.92348945, test_acc: 0.91083333, loss: 0.16717964, cum_time: 255.3675s
% With 2500 Epochs: train_acc: 0.92742224, test_acc: 0.90916667, loss: 0.16363100, cum_time: 319.2398s
% With 3000 Epochs: train_acc: 0.92920987, test_acc: 0.91000000, loss: 0.16012599, cum_time: 383.0904s
% With 3500 Epochs: train_acc: 0.92956739, test_acc: 0.91250000, loss: 0.15310866, cum_time: 446.9563s
% With 4000 Epochs: train_acc: 0.92813729, test_acc: 0.90916667, loss: 0.15610989, cum_time: 511.0209s
% Preset Learning Rate: 2e-05
% **************** NAG-m ****************
% Epoch #4050. Train_acc: 0.95816947, Test_acc: 0.93166667, Time: 0.16263890, Loss:   0.10183656
%     >>> Completed! Training time: 530.18110371
% With  500 Epochs: train_acc: 0.90060779, test_acc: 0.88333333, loss: 0.24333608, cum_time:  65.1722s
% With 1000 Epochs: train_acc: 0.92098677, test_acc: 0.90250000, loss: 0.18687027, cum_time: 130.3868s
% With 1500 Epochs: train_acc: 0.92849482, test_acc: 0.90833333, loss: 0.17537927, cum_time: 195.9024s
% With 2000 Epochs: train_acc: 0.95066142, test_acc: 0.92500000, loss: 0.11409331, cum_time: 261.4143s
% With 2500 Epochs: train_acc: 0.95352163, test_acc: 0.92416667, loss: 0.11002064, cum_time: 326.8661s
% With 3000 Epochs: train_acc: 0.95566679, test_acc: 0.93083333, loss: 0.10847763, cum_time: 392.3214s
% With 3500 Epochs: train_acc: 0.95745442, test_acc: 0.93000000, loss: 0.10141037, cum_time: 457.9370s
% With 4000 Epochs: train_acc: 0.95852699, test_acc: 0.93416667, loss: 0.09854194, cum_time: 523.4602s
% Preset Learning Rate: 2e-05
% **************** AdaGrad ****************
% Epoch #4050. Train_acc: 0.93278513, Test_acc: 0.92250000, Time: 0.11562920, Loss:   1.88231758
%     >>> Completed! Training time: 520.03005099
% With  500 Epochs: train_acc: 0.87665356, test_acc: 0.87250000, loss: 6.57001642, cum_time:  64.0983s
% With 1000 Epochs: train_acc: 0.89095459, test_acc: 0.88500000, loss: 4.82823708, cum_time: 128.2905s
% With 1500 Epochs: train_acc: 0.90811584, test_acc: 0.90250000, loss: 3.80803372, cum_time: 192.4912s
% With 2000 Epochs: train_acc: 0.91169110, test_acc: 0.90916667, loss: 3.32878803, cum_time: 256.6432s
% With 2500 Epochs: train_acc: 0.92170182, test_acc: 0.91916667, loss: 2.59969142, cum_time: 320.8391s
% With 3000 Epochs: train_acc: 0.92384698, test_acc: 0.91916667, loss: 2.46212826, cum_time: 385.1821s
% With 3500 Epochs: train_acc: 0.92956739, test_acc: 0.92000000, loss: 2.02401638, cum_time: 449.2975s
% With 4000 Epochs: train_acc: 0.93421523, test_acc: 0.92166667, loss: 1.89840887, cum_time: 513.4645s
% Preset Learning Rate: 0.0002
% **************** Adam ****************
% Epoch #4050. Train_acc: 0.98462639, Test_acc: 0.96750000, Time: 0.16235495, Loss:   0.22356477
%     >>> Completed! Training time: 555.62254095
% With  500 Epochs: train_acc: 0.95995710, test_acc: 0.94583333, loss: 1.42301104, cum_time:  68.2959s
% With 1000 Epochs: train_acc: 0.98033607, test_acc: 0.95916667, loss: 0.37027561, cum_time: 136.8379s
% With 1500 Epochs: train_acc: 0.97926350, test_acc: 0.96083333, loss: 0.56791692, cum_time: 205.2724s
% With 2000 Epochs: train_acc: 0.98033607, test_acc: 0.96583333, loss: 0.38432491, cum_time: 273.9625s
% With 2500 Epochs: train_acc: 0.89560243, test_acc: 0.90583333, loss: 4.74537381, cum_time: 342.5084s
% With 3000 Epochs: train_acc: 0.99320701, test_acc: 0.97250000, loss: 0.18040264, cum_time: 411.1799s
% With 3500 Epochs: train_acc: 0.97032535, test_acc: 0.95833333, loss: 1.20476075, cum_time: 479.9347s
% With 4000 Epochs: train_acc: 0.98998927, test_acc: 0.97166667, loss: 0.19358807, cum_time: 548.5122s
% Preset Learning Rate: 0.0002
% **************** Nadam ****************
% Epoch #4050. Train_acc: 0.97819092, Test_acc: 0.95916667, Time: 0.15214086, Loss:   0.65738586
%     >>> Completed! Training time: 528.16927195
% With  500 Epochs: train_acc: 0.84662138, test_acc: 0.82000000, loss: 18.68119302, cum_time:  65.0797s
% With 1000 Epochs: train_acc: 0.71219163, test_acc: 0.70083333, loss: 66.58093493, cum_time: 130.3231s
% With 1500 Epochs: train_acc: 0.67786915, test_acc: 0.66083333, loss: 93.66729979, cum_time: 195.5171s
% With 2000 Epochs: train_acc: 0.87415088, test_acc: 0.84250000, loss: 14.68332142, cum_time: 260.7265s
% With 2500 Epochs: train_acc: 0.91240615, test_acc: 0.89333333, loss: 9.01903476, cum_time: 325.8903s
% With 3000 Epochs: train_acc: 0.92241688, test_acc: 0.90416667, loss: 4.01285068, cum_time: 391.1688s
% With 3500 Epochs: train_acc: 0.96925277, test_acc: 0.95916667, loss: 1.01059982, cum_time: 456.3708s
% With 4000 Epochs: train_acc: 0.69074008, test_acc: 0.68083333, loss: 65.32796300, cum_time: 521.4909s
% Preset Learning Rate: 0.0002

\begin{table}[!t]
    \caption{Training accuracy achieved for continuous online training.}
    \begin{center}
        \begin{tabular}{cccccc}
            \hline
            \multirow{2}{*}{\textbf{Algorithm}} & \textbf{Learning Rate} & \multicolumn{4}{c}{\textbf{Number of Epochs}} \\
            \cline{3-6} 
             & $\eta$ & \textbf{\textit{500}}& \textbf{\textit{1000}} & \textbf{\textit{1500}} & \textbf{\textit{2000}} \\
            \hline
            SGD     & 0.00002 & 0.8702 & 0.8927 & 0.9002 & 0.9099 \\
            NAG     & 0.00002 & 0.9031 & 0.9145 & 0.9209 & 0.9234 \\
            SGD-m   & 0.00002 & 0.8802 &  0.9159 & 0.9234 & 0.9299 \\
            NAG-m   & 0.00002 & 0.9006 & 0.9209 & 0.9284 & 0.9506 \\ \hline
            AdaGrad & 0.00002 & 0.8766 & 0.8909 & 0.9081 & 0.9116 \\
            Adam    & 0.00002 & 0.9599 & 0.9803 & 0.9792 & 0.9803 \\
            Nadam   & 0.00002 & 0.8466 & 0.7121 & 0.6778 & 0.8741 \\ \hline
        \end{tabular}
        \label{tab::acc_vs_epochs_train}
    \end{center}
\end{table}

\begin{table}[!t]
    \caption{Testing accuracy achieved for continuous online training.}
    \begin{center}
        \begin{tabular}{cccccc}
            \hline
            \multirow{2}{*}{\textbf{Algorithm}} & \textbf{Learning Rate} & \multicolumn{4}{c}{\textbf{Number of Epochs}} \\
            \cline{3-6} 
             & $\eta$ & \textbf{\textit{500}}& \textbf{\textit{1000}} & \textbf{\textit{1500}} & \textbf{\textit{2000}} \\
            \hline
            SGD     & 0.00002 & 0.8383 & 0.8683 & 0.8808 & 0.8891 \\
            NAG     & 0.00002 & 0.8875 & 0.8933 & 0.9041 & 0.9108 \\
            SGD-m   & 0.00002 & 0.8691 & 0.9033 & 0.9091 & 0.9108 \\
            NAG-m   & 0.00002 & 0.8833 & 0.9025 & 0.9083 & 0.9250 \\ \hline
            AdaGrad & 0.00002 & 0.8725 & 0.8850 & 0.9025 & 0.9091 \\
            Adam    & 0.00002 & 0.9458 & 0.9591 & 0.9608 & 0.9658 \\
            Nadam   & 0.00002 & 0.8200 & 0.7008 & 0.6608 & 0.8425 \\ \hline
        \end{tabular}
    \label{tab::acc_vs_epochs_test}
    \end{center}
\end{table}

% \begin{table}[!t]
%     \caption{Training accuracy achieved for continuous online training.}
%     \begin{center}
%         \begin{tabular}{cccccc}
%             \hline
%             \multirow{2}{*}{\textbf{Algorithm}} & \textbf{Learning Rate} & \multicolumn{4}{c}{\textbf{Number of Epochs}} \\
%             \cline{3-6} 
%              & $\eta$ & \textbf{\textit{500}}& \textbf{\textit{1000}} & \textbf{\textit{1500}} & \textbf{\textit{2000}} \\
%             \hline
%             SGD     & 0.00002 &
%             NAG     & 0.00002 &  &  &  & \\
%             SGD-m   & 0.00002 &  &  &  & \\
%             NAG-m   & 0.00002 &  &  &  & \\ \hline
%             AdaGrad & 0.00002 &  &  &  & \\
%             Adam    & 0.00002 &  &  &  &  \\
%             Nadam   & 0.00002 &  &  &  & \\ \hline
%         \end{tabular}
%         \label{tab::acc_vs_epochs_train}
%     \end{center}
% \end{table}


% \begin{table}[!t]
%     \caption{Testing accuracy achieved for continuous online training.}
%     \begin{center}
%         \begin{tabular}{cccccc}
%             \hline
%             \multirow{2}{*}{\textbf{Algorithm}} & \textbf{Learning Rate} & \multicolumn{4}{c}{\textbf{Number of Epochs}} \\
%             \cline{3-6} 
%              & $\eta$ & \textbf{\textit{500}}& \textbf{\textit{1000}} & \textbf{\textit{1500}} & \textbf{\textit{2000}} \\
%             \hline
%             SGD     & 0.00002 &  &  &  & \\
%             NAG     & 0.00002 &  &  &  & \\
%             SGD-m   & 0.00002 &  &  &  & \\
%             NAG-m   & 0.00002 &  &  &  & \\ \hline
%             AdaGrad & 0.00002 &  &  &  & \\
%             Adam    & 0.00002 &  &  &  &  \\
%             Nadam   & 0.00002 &  &  &  & \\ \hline
%         \end{tabular}
%     \label{tab::acc_vs_epochs_test}
%     \end{center}
% \end{table}


==> test_results_old.tex <==
\begin{table}[!t]
    \caption{Training accuracy achieved for continuous online training.}
    \begin{center}
        \begin{tabular}{cccccc}
            \hline
            \multirow{2}{*}{\textbf{Algorithm}} & \textbf{Learning Rate} & \multicolumn{4}{c}{\textbf{Number of Epochs}} \\
            \cline{3-6} 
             & $\eta$ & \textbf{\textit{1000}}& \textbf{\textit{2000}} & \textbf{\textit{3000}} & \textbf{\textit{4000}} \\
            \hline
            SGD     & 0.00002 & 0.8653 & 0.8986 & 0.9095 & 0.9228 \\
            NAG     & 0.00002 & 0.8890 & 0.9040 & 0.9178 & 0.9241 \\
            SGD-m   & 0.00002 & 0.8986 & 0.9140 & 0.9286 & 0.9353 \\
            NAG-m   & 0.00002 & 0.8886 & 0.9203 & 0.9278 & 0.9353 \\ \hline
            AdaGrad & 0.00002 & 0.3636 & 0.7543 & 0.7839 & 0.8035 \\
            Adam    & 0.00002 & 0.9378 & 0.9658 & 0.9812 & 0.9883  \\
            Nadam   & 0.00002 & 0.9241 & 0.9186 & 0.9532 & 0.9728 \\ \hline
        \end{tabular}
        \label{tab::acc_vs_epochs_train}
    \end{center}
\end{table}


\begin{table}[!t]
    \caption{Testing accuracy achieved for continuous online training.}
    \begin{center}
        \begin{tabular}{cccccc}
            \hline
            \multirow{2}{*}{\textbf{Algorithm}} & \textbf{Learning Rate} & \multicolumn{4}{c}{\textbf{Number of Epochs}} \\
            \cline{3-6} 
             & $\eta$ & \textbf{\textit{1000}}& \textbf{\textit{2000}} & \textbf{\textit{3000}} & \textbf{\textit{4000}} \\
            \hline
            SGD     & 0.00002$^{\mathrm{a}}$ & 0.8405 & 0.8861 & 0.8999 & 0.9111 \\
            NAG     & 0.00002$^{\mathrm{a}}$ & 0.8755 & 0.8961 & 0.9036 & 0.9118 \\
            SGD-m   & 0.00002$^{\mathrm{a}}$ & 0.8636 & 0.8836 & 0.8999 & 0.9043 \\
            NAG-m   & 0.00002$^{\mathrm{a}}$ & 0.8786 & 0.9024 & 0.9080 & 0.9174 \\ \hline
            AdaGrad & 0.00002 & 0.3589 & 0.7348 & 0.7698 & 0.7936  \\
            Adam    & 0.00002 & 0.9061 & 0.9343 & 0.9462 & 0.9555  \\
            Nadam   & 0.00002 & 0.9111 & 0.9068 & 0.9274 & 0.9399  \\ \hline
            AdaGrad & 0.0002  & 0.8486 & 0.8755 & 0.8836 & 0.8924  \\
            Adam    & 0.0002  & 0.9555 & 0.9537 & 0.9599 & 0.9681  \\
            Nadam   & 0.0002  & 0.8911 & 0.9412 & 0.8792 & 0.9043  \\ \hline
        \end{tabular}
    \label{tab::acc_vs_epochs_test}
    \end{center}
\end{table}


\begin{table*}[!t] % DELETE LATER
    \caption{Computational Performances in time elapsed (seconds).}
    \begin{center}
        \begin{tabular}{cc||cccc|cccc}
            \hline
            \multirow{3}{*}{\textbf{Algorithm}} & \multirow{3}{*}{\textbf{Learning Rate}} & \multicolumn{8}{c}{\textbf{Computational Platform}} \\
            \cline{3-10} 
             & & \multicolumn{4}{c|}{\textbf{\textit{CPU}}} & \multicolumn{4}{c}{\textbf{\textit{GPU}}}  \\
            \cline{3-10} 
             & & \textbf{\textit{1000}} & \textbf{\textit{2000}} & \textbf{\textit{3000}} & \textbf{\textit{4000}} & \textbf{\textit{1000}} & \textbf{\textit{2000}} & \textbf{\textit{3000}} & \textbf{\textit{4000}}  \\ \hline
            SGD     & 0.00002 & & & & & 125.26 & 250.15 & 375.02 & 500.04  \\
            NAG     & 0.00002 & & & & & 124.59 & 249.30 & 374.26 & 499.28  \\
            SGD-m   & 0.00002 & & & & & 132.94 & 266.09 & 399.35 & 532.23 \\
            NAG-m   & 0.00002 & & & & & 125.30 & 250.76 & 375.94 & 501.27 \\ \hline
            AdaGrad & 0.0002  & & & & & 124.98 & 250.25 & 375.73 & 501.34 \\
            Adam    & 0.0002  & & & & & 134.57 & 269.34 & 404.13 & 538.87 \\
            Nadam   & 0.0002  & & & & & 128.67 & 257.74 & 386.75 & 515.71 \\ \hline
            AdaGrad & 0.00002 & & & & & 128.85 & 259.29 & 389.55 & 518.17 \\
            Adam    & 0.00002 & & & & & 138.68 & 277.35 & 416.05 & 554.80 \\
            Nadam   & 0.00002 & & & & & 132.25 & 264.53 & 397.23 & 529.63 \\ \hline
        \end{tabular}
    \label{tab::cmpt_perform}
    \end{center}
\end{table*}

